LogStamp: Automatic Online Log Parsing Based on Sequence Labelling

Logs are one of the most critical data for service management. It contains rich runtime information for both services and users. Since size of logs are often enormous in size and have free handwritten constructions, a typical log-based analysis needs to parse logs into structured format first. However, we observe that most existing log parsing methods cannot parse logs online, which is essential for online services. In this paper, we present an automatic online log parsing method, name as LogStamp. We extensively evaluate LogStamp on five public datasets to demonstrate the effectiveness of our proposed method. The experiments show that our proposed method can achieve high accuracy with only a small portion of the training set. For example, it can achieve an average accuracy of 0.956 when using only 10% of the data training.

==> acknowledgment.tex <==
We thank the anonymous reviewers for their valuable feedback. 

==> figures/name.tex <==
import math
import string
import json
import re
import base64
import time
from datetime import datetime

remove_list = ['pred_single','index',
               'request_content_length',
               # 'behinder_user_agent',
               # 'response_content_length', 'request_behinder_score',
               # 'request_gsl_score'
]  #'request_body_is_base64', 'response_body_is_base64',
replace = {'True': True, 'False': False, '': 0.0}

normal_dict = {'request_header': 101, 'http_method': 29,
                   'response_header': 103, 'request_body': 102,
                   'response_body': 104, 'request_length': 81, 'response_length': 82}
# anomalous_dict = {'request_header':85, 'http_method':29, 'response_header':87, 'request_body':86, 'response_body':88}
white_dict = {'request_header': 0, 'http_method': 4, 'response_header': 2, 'request_body': 1,
              'response_body': 3}  # input_type=1
map_dict = {0: normal_dict, 1: white_dict}

#### 统计的类别
order_list = [
        'pred_single',
        'index',
        'request_has_pragma', 'request_pragma_is_no_cache',
        'request_has_cache_pragma',
        'request_has_cache_control', 'request_cache_is_no_cache',
        'request_accept_word_length', 'request_accept_string_length',
        'response_has_cache_control',  'response_is_no_store_must',
        'response_has_cache_pragma',
        'response_has_pragma','response_pragma_is_no_cache',
        'request_body_is_base64', 'response_body_is_base64',
        # 'request_body_entropy', 'request_body_CI',
        # 'response_body_entropy','response_body_CI',
        'request_keep_alive', 'response_keep_alive',
        'behinder_user_agent','response_content_type',
        'http_method_is_post','request_content_length', 'response_content_length',
        'response_transfer_encoding',
        'request_behinder_score', 'response_behinder_score',
        'request_gsl_score', 'response_gsl_score',
        'response_behinder_jsp_score', 'response_gsl_jsp_score',
        'request_content_length_is_last',
        'response_content_type_is_last',
        # 'session_semicolon',
        'content_type_texthtml',

    ]

def is_base64_code(s):
    '''判断是否是base64'''
    if not isinstance(s, str) or not s:
        # print("params s not string or None")
        return False

    _base64_code = ['A', 'B', 'C', 'D', 'E', 'F', 'G', 'H', 'I',
                    'J', 'K', 'L', 'M', 'N', 'O', 'P', 'Q', 'R',
                    'S', 'T', 'U', 'V', 'W', 'X', 'Y', 'Z', 'a',
                    'b', 'c', 'd', 'e', 'f', 'g', 'h', 'i', 'j',
                    'k', 'l', 'm', 'n', 'o', 'p', 'q', 'r', 's',
                    't', 'u', 'v', 'w', 'x', 'y', 'z', '0', '1',
                    '2', '3', '4', '5', '6', '7', '8', '9', '+',
                    '/', '=']

    # Check base64 OR codeCheck % 4
    code_fail = [i for i in s if i not in _base64_code]
    if code_fail or len(s) % 4 != 0:
        return False
    return True


def cal_entropy(text):
    '''
    计算信息熵
    :param text:
    :return:
    '''

    h = 0.0
    sum = 0
    letter = [0] * 26
    text = text.lower()
    for i in range(len(text)):
        if text[i].isalpha():
            letter[ord(text[i]) - ord('a')] += 1
            sum += 1
    # print('\n', letter)
    if sum == 0:
        return 0
    for i in range(26):
        p = 1.0 * letter[i] / sum
        if p > 0:
            h += -(p * math.log(p, 2))
    return h


def cal_coincidence_index(text):
    '''
    计算重合指数  Index of Coincidence
    :param text:
    :return:
    '''
    lowercase = string.ascii_lowercase

    def get_trim_text(text):
        text = text.lower()
        trim_text = ''
        for l in text:
            if lowercase.find(l) >= 0:
                trim_text += l
        return trim_text

    trim_text = get_trim_text(text)
    length = len(trim_text)
    letter_stats = []
    for l in lowercase:
        lt = {}
        count = trim_text.count(l)
        lt[l] = count
        letter_stats.append(lt)

    index = 0
    if length == 0:
        return 0
    for d in letter_stats:
        v = list(d.values())[0]
        index += (v / length) ** 2

    return index


def head_to_json(head):
    head_dict = {}
    # 按字段分隔
    head_list_middle = re.split(r'\r|\n|\\r|\\n', head)
    head_list = [n for n in head_list_middle if n]
    # 获取key-value,保存成字典
    for item in head_list:
        # 避免数据中没有:或者数据不全
        if ":" in item:
            key, value = item.split(':', 1)
            key = key.lower()
            head_dict[key.strip()] = value.strip()
    # 转换成json
    json_str = json.dumps(head_dict)
    return json_str


def head_to_dict(head):
    head_dict = {}
    head_order = []
    # 按字段分隔
    head_list_middle = re.split(r'\r|\n|\\r|\\n', head)
    head_list = [n for n in head_list_middle if n]
    # 获取key-value,保存成字典
    for item in head_list:
        # 避免数据中没有:或者数据不全
        if ":" in item:
            key, value = item.split(':', 1)
            key = key.lower()
            # print(key)
            head_dict[key.strip()] = value.strip()
            head_order.append(key.strip())
    return head_dict, head_order


def get_accept_length(head_dict):
    # 不存在则为0
    accept_word_length = 0
    accept_string_length = 0
    # print(head_dict)
    if 'accept' in head_dict.keys():
        accept_string_length = len(head_dict['accept'])
        accept_list = re.split(',|;', head_dict['accept'])
        accept_word_length = len(accept_list)
    return accept_word_length, accept_string_length


def get_cache_control(head_dict):
    has_cache_control = False
    is_no_cache = False
    is_no_store_must = False
    if 'cache-control' in head_dict.keys():
        has_cache_control = True
        # 某子串是否存在于字符串，直接使用in
        if "no-cache" in head_dict['cache-control']:
            is_no_cache = True
        if "no-store, no-cache, must-revalidate" in head_dict['cache-control']:
            is_no_store_must = True
    return has_cache_control, is_no_cache, is_no_store_must


def get_cache_pragma(head_dict):
    has_cache_pragma = False
    if 'pragma' in head_dict.keys() and 'cache-control' in head_dict.keys():
        has_cache_pragma = True
    return has_cache_pragma


def find_pragma(header_dict):
    '''
    判断header中是否包含pregma，若包含再判断是否包含no-cache值
    :param head_dict: 字典型的header
    :return: 两个bool型的返回值，分别代表是否包含pregma及是否包含no-cache值
    '''
    has_pragma = False
    is_no_cache = False
    if 'pragma' in header_dict.keys():
        has_pragma = True
        if header_dict['pragma'] == "no-cache":
            is_no_cache = True
    return has_pragma, is_no_cache


def find_keep_alive(header_dict):
    has_keep_alive = False
    if 'connection' in header_dict.keys():
        if header_dict['connection'].lower() == 'keep-alive':
            has_keep_alive = True
    return has_keep_alive


def find_user_agent_behinder(header_dict):
    # 目前是24个user agent
    ua = [
        "Mozilla/5.0 (Windows NT 10.0; Win64; x64; rv:84.0) Gecko/20100101",
        "Mozilla/5.0 (Windows NT 10.0; Win64; x64; rv:79.0) Gecko/20100101 Firefox/79.0",
        "Mozilla/5.0 (Macintosh; Intel Mac OS X 10.15; rv:79.0) Gecko/20100101 Firefox/79.0",
        "Mozilla/5.0 (X11; Linux i686; rv:79.0) Gecko/20100101 Firefox/79.0",
        "Mozilla/5.0 (Linux x86_64; rv:79.0) Gecko/20100101 Firefox/79.0",
        "Mozilla/5.0 (X11; Ubuntu; Linux i686; rv:79.0) Gecko/20100101 Firefox/79.0",
        "Mozilla/5.0 (X11; Ubuntu; Linux x86_64; rv:79.0) Gecko/20100101 Firefox/79.0",
        "Mozilla/5.0 (X11; Fedora; Linux x86_64; rv:79.0) Gecko/20100101 Firefox/79.0",
        "Mozilla/5.0 (compatible; MSIE 10.0; Windows NT 6.1; WOW64; Trident/6.0)",
        "Mozilla/5.0 (compatible; MSIE 10.0; Windows NT 6.2)",
        "Mozilla/5.0 (Windows NT 6.1; Trident/7.0; rv:11.0) like Gecko",
        "Mozilla/5.0 (Windows NT 6.2; Trident/7.0; rv:11.0) like Gecko",
        "Mozilla/5.0 (Windows NT 6.3; Trident/7.0; rv:11.0) like Gecko",
        "Mozilla/5.0 (Macintosh; Intel Mac OS X 10_13_6) AppleWebKit/537.36 (KHTML, like Gecko) Chrome/84.0.4147.125 Safari/537.36",
        "Mozilla/5.0 (Macintosh; Intel Mac OS X 10_13_6) AppleWebKit/605.1.15 (KHTML, like Gecko) Version/13.1.2 Safari/605.1.15",
        "Mozilla/5.0 (Windows NT 10.0; Win64; x64) AppleWebKit/537.36 (KHTML, like Gecko) Chrome/84.0.4147.125 Safari/537.36",
        "Mozilla/5.0 (Windows NT 10.0; WOW64) AppleWebKit/537.36 (KHTML, like Gecko) Chrome/84.0.4147.125 Safari/537.36",
        "Mozilla/5.0 (Windows NT 10.0) AppleWebKit/537.36 (KHTML, like Gecko) Chrome/84.0.4147.125 Safari/537.36",
        "Mozilla/5.0 (Macintosh; Intel Mac OS X 10_15_6) AppleWebKit/537.36 (KHTML, like Gecko) Chrome/84.0.4147.125 Safari/537.36",
        "Mozilla/5.0 (X11; Linux x86_64) AppleWebKit/537.36 (KHTML, like Gecko) Chrome/84.0.4147.125 Safari/537.36",
        "Mozilla/5.0 (iPhone; CPU iPhone OS 13_6 like Mac OS X) AppleWebKit/605.1.15 (KHTML, like Gecko) CriOS/84.0.4147.122 Mobile/15E148 Safari/604.1",
        "Mozilla/5.0 (iPad; CPU OS 13_6 like Mac OS X) AppleWebKit/605.1.15 (KHTML, like Gecko) CriOS/84.0.4147.122 Mobile/15E148 Safari/604.1",
        "Mozilla/5.0 (iPod; CPU iPhone OS 13_6 like Mac OS X) AppleWebKit/605.1.15 (KHTML, like Gecko) CriOS/84.0.4147.122 Mobile/15E148 Safari/604.1",
        "Mozilla/5.0 (Linux; Android 10) AppleWebKit/537.36 (KHTML, like Gecko) Chrome/84.0.4147.125 Mobile Safari/537.36",
        "Mozilla/5.0 (Macintosh; Intel Mac OS X 10_15_6) AppleWebKit/537.36 (KHTML, like Gecko) Chrome/84.0.4147.125 Safari/537.36",
        "Mozilla/5.0 (iPhone; CPU iPhone OS 13_6 like Mac OS X) AppleWebKit/605.1.15 (KHTML, like Gecko) CriOS/84.0.4147.122 Mobile/15E148 Safari/604.1",
    ]
    user_agent = False
    if 'user-agent' in header_dict.keys():
        # print(header_dict['user-agent'])
        if header_dict['user-agent'] in ua:
            user_agent = True
    return user_agent


def get_content_type(header_dict):
    response_content_type = False
    if 'content-type' in header_dict.keys():
        if header_dict['content-type'].lower() == 'text/html; charset=utf-8':
            response_content_type = True
    return response_content_type


def get_content_type_html(header_dict):
    response_content_type = False
    if 'content-type' in header_dict.keys():
        if header_dict['content-type'].lower() == 'text/html':
            response_content_type = True
    return response_content_type


def check_http_post(method):
    is_post = False
    if method.lower() == 'post':
        is_post = True
    return is_post


def get_content_length(header_dict, http_body):
    content_length = 0
    if 'content-length' in header_dict.keys():
        content_length = header_dict['content-length']
    else:
        new_http_body = http_body
        if is_base64_code(http_body):
            try:
                new_http_body = base64.b64decode(http_body).decode()
            except:
                new_http_body = http_body
        content_length = len(new_http_body)
    return str(content_length)


def transfer_encoding(header_dict):
    '''
    冰蝎3.0 连续的第二组response没有content-length、包含connection:keep-alive和 Transfer-Encoding:chunked
    :param header_dict:
    :return:
    '''
    response_transfer_encoding = False
    if 'content-length' not in header_dict.keys():
        if 'connection' in header_dict.keys() and header_dict['connection'].lower() == 'keep-alive':
            if 'transfer-encoding' in header_dict.keys() and header_dict['transfer-encoding'].lower() == 'chunked':
                response_transfer_encoding = True
    return response_transfer_encoding


def lcs(s1, s2):
    # 生成0矩阵，为方便后续计算，比字符串长度多了一列
    m = [[0 for i in range(len(s2) + 1)] for j in range(len(s1) + 1)]
    # 最长匹配的长度
    mmax = 0
    # 最长匹配对应在s1中的最后一位
    p = 0
    for i in range(len(s1)):
        for j in range(len(s2)):
            # 如果相等，则加入现有的公共子串
            if s1[i] == s2[j]:
                m[i + 1][j + 1] = m[i][j] + 1
                if m[i + 1][j + 1] > mmax:
                    mmax = m[i + 1][j + 1]
                    p = i + 1
    # 返回最长子串及其长度
    return s1[p - mmax:p], mmax


def get_header_lcs(head_list, flag='request'):
    map = {'accept': 'a', 'accept-encoding': 'b', 'accept-language': 'c',
           'content-type': 'd', 'referer': 'e', 'user-agent': 'f',
           'cache-control': 'g', 'pragma': 'h', 'host': 'i',
           'connection': 'g', 'content-length': 'k', 'server': 'l',
           'x-powered-by': 'm', 'expires': 'n', 'keep-alive': 'o',
           'transfer-encoding': 'p', 'cookie': 'q', 'set-cookie': 'r',
           'date': 's',
           }

    cur_order = [map[i] for i in head_list if i in map]
    if flag == 'request':
        # 冰蝎3.0 php/jsp
        behinder = ['accept', 'accept-encoding', 'accept-language', 'content-type', 'referer', 'user-agent',
                    'cache-control', 'pragma', 'host', 'connection', 'content-length', 'cookie']
        behinder_order = [map[i] for i in behinder if i in map]
        # 哥斯拉 php/jsp
        gsl = ['user-agent', 'accept', 'accept-language', 'host', 'connection', 'content-type', 'content-length']
        gsl_order = [map[i] for i in gsl if i in map]


        behinder_str, behinder_len = lcs(behinder_order, cur_order)
        gsl_str, gsl_len = lcs(gsl_order, cur_order)
        if len(head_list) == 0:
            return 0, 0, 0, 0
        else:
            behinder_score = behinder_len / len(head_list)
            gsl_score = gsl_len / len(head_list)
        return behinder_score, gsl_score, 0, 0

        # response
    else:
        behinder = ['server', 'x-powered-by', 'expires', 'cache-control', 'pragma', 'content-length',
                    'keep-alive', 'connection', 'transfer-encoding', 'content-type']
        # behinder =[]

        behinder_order = [map[i] for i in behinder if i in map]

        gsl = ['server', 'x-powered-by', 'expires', 'cache-control', 'pragma', 'content-length',
               'keep-alive', 'connection', 'content-type']
        gsl_order = [map[i] for i in gsl if i in map]

        behinder_jsp = [ 'content-type','transfer-encoding', 'Date',  'keep-alive', 'connection']
        behinder_jsp_order = [map[i] for i in behinder_jsp if i in map]

        gsl_jsp = [ 'content-type','content-length','Date', 'keep-alive', 'connection']
        gsl_jsp_order = [map[i] for i in gsl_jsp if i in map]

        behinder_str, behinder_len = lcs(behinder_order, cur_order)
        gsl_str, gsl_len = lcs(gsl_order, cur_order)
        behinder_jsp_str, behinder_jsp_len = lcs(behinder_jsp_order, cur_order)
        gsl_jsp_str, gsl_jsp_len = lcs(gsl_jsp_order, cur_order)
        if len(head_list) == 0:
            return 0, 0, 0, 0
        else:
            behinder_score = behinder_len / len(head_list)
            gsl_score = gsl_len / len(head_list)
            behinder_jsp_score = behinder_jsp_len / len(head_list)
            gsl_jsp_score = gsl_jsp_len / len(head_list)

        return behinder_score, gsl_score, behinder_jsp_score, gsl_jsp_score


def extract_features(line, count_list,  input_type=0, is_csv=True, remove_null=True  ):
    '''

    :param line:
    :param input_type:
    :param is_csv:
    :param remove_null:
    :param count_list: [total, error, count_null,behinder, godzilla]
    :return:
    '''
    index_dict = map_dict[input_type]
    count_dict = {}
    for item in order_list:
        count_dict[item] = []

    if is_csv:
        l = line.strip().split(',')
    else:
        l = line.strip().split('^')
    l = [d.replace('"', '') for d in l]

    # 跳过不规整的行
    if len(l) < 5:
        # 表示没有处理就return了
        # print('len(l) < 5')
        return -1

    count_list[0] += 1

    try:
        http_method = l[index_dict['http_method']]
        request_header = base64.b64decode(l[index_dict['request_header']]).decode()

        request_header_dict, request_header_list = head_to_dict(request_header)

        response_header = base64.b64decode(l[index_dict['response_header']]).decode()
        response_header_dict, response_header_list = head_to_dict(response_header)

        request_body = l[index_dict['request_body']]
        response_body = l[index_dict['response_body']]

        if request_header == '' or response_header == '':
            if remove_null:
                count_list[2] += 1
                # 表示没有处理就return了
                return -1

        # print(request_header)
                # print('http_method',http_method)
                # print('request_header',request_header)
                # print('response_header',response_header)
                # print('request_body',request_body)
                # print('response_body',response_body)
                # print()
    except Exception as e:
        # print("!!!!Exception utils.extract_features():", e)
        count_list[1] += 1
        return -1
    extract_features
    count_dict['index'].append(count_list[0])
    #####################################################
    #### ↓↓↓下面堆加 request header 的判断函数↓↓↓##
    #####################################################
    # 判断content-length是否是最后一个
    content_length_is_last = last_content_length(request_header_list)
    count_dict['request_content_length_is_last'].append(content_length_is_last)

    # 计算header的顺序相似度
    request_behinder_score, request_gsl_score, _, _ = get_header_lcs(request_header_dict, 'request')
    count_dict['request_behinder_score'].append(request_behinder_score)
    count_dict['request_gsl_score'].append(request_gsl_score)

    # 统计content-length
    if input_type == 0:
        request_content_length = l[index_dict['request_length']]
    else:
        request_content_length = get_content_length(request_header_dict, request_body)
    count_dict['request_content_length'].append(request_content_length)

    # 判断http method是否是post
    http_method_is_post = check_http_post(http_method)
    count_dict['http_method_is_post'].append(http_method_is_post)

    # 判断user agent是否命中冰蝎
    behinder_user_agent = find_user_agent_behinder(request_header_dict)
    count_dict['behinder_user_agent'].append(behinder_user_agent)

    # 判断是否Connection: keep-alive
    request_keep_alive = find_keep_alive(request_header_dict)
    count_dict['request_keep_alive'].append(request_keep_alive)

    # 判断是否具有pragma, 是否包含no-cache
    request_has_pragma, request_pragma_is_no_cache = find_pragma(request_header_dict)
    count_dict['request_has_pragma'].append(request_has_pragma)
    count_dict['request_pragma_is_no_cache'].append(request_pragma_is_no_cache)

    # 判断是否同时具有cache control 和pragma
    request_has_cache_pragma = get_cache_pragma(request_header_dict)
    count_dict['request_has_cache_pragma'].append(request_has_cache_pragma)

    # 判断是否具有cache_control，是否包含no-cache值和no-store, no-cache, must-revalidate
    request_has_cache_control, request_cache_is_no_cache, _ = get_cache_control(request_header_dict)
    count_dict['request_has_cache_control'].append(request_has_cache_control)
    count_dict['request_cache_is_no_cache'].append(request_cache_is_no_cache)
    # count_dict['request_is_no_store_must'].append(request_is_no_store_must)

    # 计算accept的长度, 包括按照逗号或者分号分隔后的数量以及字符串长度
    request_accept_word_length, request_accept_string_length = get_accept_length(request_header_dict)
    count_dict['request_accept_word_length'].append(request_accept_word_length)
    count_dict['request_accept_string_length'].append(request_accept_string_length)

    #####################################################
    #### ↓↓↓下面堆加 response header 的判断函数↓↓↓#
    #####################################################
    # #判断session后面时候有分号
    # session_semicolon =  find_session_semicolon(response_header_dict)
    # count_dict['session_semicolon'].append(session_semicolon)

    # # 判断content-type是否是最后一个
    response_content_type_is_last = last_content_type(response_header_list)
    count_dict['response_content_type_is_last'].append(response_content_type_is_last)

    # 计算header顺序相似度
    response_behinder_score, response_gsl_score, response_behinder_jsp_score, response_gsl_jsp_score = get_header_lcs(
        response_header_dict, 'response')
    count_dict['response_behinder_score'].append(response_behinder_score)
    count_dict['response_gsl_score'].append(response_gsl_score)
    count_dict['response_behinder_jsp_score'].append(response_behinder_jsp_score)
    count_dict['response_gsl_jsp_score'].append(response_gsl_jsp_score)

    # 判断transfer-encoding:chunked
    response_transfer_encoding = transfer_encoding(response_header_dict)
    count_dict['response_transfer_encoding'].append(response_transfer_encoding)

    # 统计content-length
    if input_type == 0:
        response_content_length = l[index_dict['response_length']]
        if response_content_length == '':
            response_content_length = '0'
    else:
        response_content_length = get_content_length(response_header_dict, response_body)
        if response_content_length == '':
            response_content_length = '0'

    count_dict['response_content_length'].append(response_content_length)

    # 判断content-type是否是'text/html; charset=utf-8'
    response_content_type = get_content_type(response_header_dict)
    count_dict['response_content_type'].append(response_content_type)

    # 判断content-type是不是'text/html'
    response_content_type = get_content_type_html(response_header_dict)
    count_dict['content_type_texthtml'].append(response_content_type)

    # 判断是否Connection: keep-alive
    response_keep_alive = find_keep_alive(response_header_dict)
    count_dict['response_keep_alive'].append(response_keep_alive)

    # 判断是否具有cache_control，是否包含no-cache值和no-store, no-cache, must-revalidate
    response_has_cache_control, _, response_is_no_store_must = get_cache_control(
        response_header_dict)
    count_dict['response_has_cache_control'].append(response_has_cache_control)
    count_dict['response_is_no_store_must'].append(response_is_no_store_must)

    # 判断是否同时具有cache control 和pragma
    response_has_cache_pragma = get_cache_pragma(response_header_dict)
    count_dict['response_has_cache_pragma'].append(response_has_cache_pragma)

    # 判断是否具有pragma, 是否包含no-cache
    response_has_pragma, response_pragma_is_no_cache = find_pragma(response_header_dict)
    count_dict['response_has_pragma'].append(response_has_pragma)
    count_dict['response_pragma_is_no_cache'].append(response_pragma_is_no_cache)

    #####################################################
    #### ↓↓↓下面堆加 request body 的判断函数↓↓↓####
    #####################################################
    request_body_is_base64 = is_base64_code(request_body)
    count_dict['request_body_is_base64'].append(request_body_is_base64)

    # request_body_entropy = cal_entropy(request_body)
    # request_body_CI = cal_coincidence_index(request_body)
    # count_dict['request_body_entropy'].append(request_body_entropy)
    # count_dict['request_body_CI'].append(request_body_CI)

    #####################################################
    #### ↓↓↓下面堆加 response body 的判断函数↓↓↓###
    #####################################################
    response_body_is_base64 = is_base64_code(response_body)
    count_dict['response_body_is_base64'].append(response_body_is_base64)

    # response_body_entropy = cal_entropy(response_body)
    # response_body_CI = cal_coincidence_index(response_body)
    # count_dict['response_body_entropy'].append(response_body_entropy)
    # count_dict['response_body_CI'].append(response_body_CI)
    return count_dict

def detect_by_rules(count_dict):
    # 0:正常  1:冰蝎  2:哥斯拉
    res = 0

    request_has_pragma = count_dict['request_has_pragma'][-1]
    request_pragma_is_no_cache = count_dict['request_pragma_is_no_cache'][-1]
    request_has_cache_pragma = count_dict['request_has_cache_pragma'][-1]
    request_has_cache_control = count_dict['request_has_cache_control'][-1]
    request_cache_is_no_cache = count_dict['request_cache_is_no_cache'][-1]
    request_accept_word_length = count_dict['request_accept_word_length'][-1]
    request_accept_string_length = count_dict['request_accept_string_length'][-1]
    response_has_cache_control = count_dict['response_has_cache_control'][-1]
    response_is_no_store_must = count_dict['response_is_no_store_must'][-1]
    response_has_cache_pragma = count_dict['response_has_cache_pragma'][-1]
    response_has_pragma = count_dict['response_has_pragma'][-1]
    response_pragma_is_no_cache = count_dict['response_pragma_is_no_cache'][-1]
    request_body_is_base64 = count_dict['request_body_is_base64'][-1]
    response_body_is_base64 = count_dict['response_body_is_base64'][-1]
    request_keep_alive = count_dict['request_keep_alive'][-1]
    response_keep_alive = count_dict['response_keep_alive'][-1]
    behinder_user_agent = count_dict['behinder_user_agent'][-1]
    response_content_type = count_dict['response_content_type'][-1]
    http_method_is_post = count_dict['http_method_is_post'][-1]
    # request_content_length = count_dict['request_content_length'][-1]
    # response_content_length = count_dict['response_content_length'][-1]
    response_transfer_encoding = count_dict['response_transfer_encoding'][-1]
    request_behinder_score = count_dict['request_behinder_score'][-1]
    response_behinder_score = count_dict['response_behinder_score'][-1]
    request_gsl_score = count_dict['request_gsl_score'][-1]
    response_gsl_score = count_dict['response_gsl_score'][-1]
    request_content_length_is_last = count_dict['request_content_length_is_last'][-1]
    response_content_type_is_last = count_dict['response_content_type_is_last'][-1]

    count = request_has_pragma + request_pragma_is_no_cache + request_has_cache_pragma \
            + request_has_cache_control + request_cache_is_no_cache + response_has_cache_control \
            + response_is_no_store_must + response_has_cache_pragma + response_has_pragma \
            + request_body_is_base64 + response_body_is_base64 + request_keep_alive \
            + behinder_user_agent + response_content_type + http_method_is_post \
            + response_transfer_encoding + response_pragma_is_no_cache + response_keep_alive


    # 冰蝎
    if response_has_cache_control and response_is_no_store_must and response_has_pragma and response_pragma_is_no_cache \
            and response_content_type and request_behinder_score >= 0.3 and response_behinder_score >= 0.45:  # and response_transfer_encoding
        return 1  # 冰蝎

    # 哥斯拉
    if response_has_cache_control and response_is_no_store_must and response_has_pragma and response_pragma_is_no_cache \
            and http_method_is_post and response_content_type and response_gsl_score >= 0.45 and request_content_length_is_last:
        return 2  # 哥斯拉


    return res


# def output_to_file(output, count_dict, order_list, file_method='w'):
#     # 输出features到文件
#     f = open(output, file_method)
#     res = ''
#     if file_method == 'w':
#         for feature_name in order_list:
#             res = res + feature_name + ','
#         f.writelines(res[:-1] + '\n')
#
#     for index in range(len(count_dict[order_list[0]])):
#         res = ''
#         for feature_name in order_list:
#             # print(feature_name)
#             res = res + str(count_dict[feature_name][index]) + ','
#         f.writelines(res[:-1] + '\n')
#     f.close()
#     print('extracted features have saved to "%s"' % output)


def get_cookie(request_header_dict, response_header_dict):
    cookie = ''
    # print(head_dict)
    if 'cookie' in request_header_dict:
        # print(request_header_dict['cookie'])
        m = re.search("ID=([A-Za-z0-9]+);", request_header_dict['cookie'])
        if m:
            cookie = m.group(1)
    if 'set-cookie' in response_header_dict:
        # print(response_header_dict['set-cookie'])
        m = re.search("ID=([A-Za-z0-9]+);", response_header_dict['set-cookie'])
        if m:
            cookie = m.group(1)
    # print(cookie)
    return cookie


def get_timestamp(str_time):
    '''
    提供给Kibana进行统计的时间, 解析成数字
    :param str_time: 2021-10-25T08:43:24.663
    :return:
    '''
    datetime_obj = datetime.strptime(str_time, "%Y-%m-%dT%H:%M:%S.%f")
    ret_stamp = int(time.mktime(datetime_obj.timetuple()) * 1000.0 + datetime_obj.microsecond / 1000.0)
    # print(ret_stamp)
    return ret_stamp


def last_content_length(head_list):
    # print('head_list', head_list)
    if len(head_list) < 2:
        return False
    if head_list[-1] == 'content-length':
        return True
    else:
        return False


def last_content_type(head_list):
    # print('head_list', head_list)
    if len(head_list) < 2:
        return False
    if head_list[-1] == 'content-type':
        return True
    else:
        return False


def find_session_semicolon(head_dict):
    if 'cookie' in head_dict:
        # print(head_dict['cookie'])
        m = re.search("PHPSESSID=66qepujvqe1lksqkj2koosfke7;", head_dict['cookie'])
        if m:
            print(head_dict)
            return True
    if 'set-cookie' in head_dict:
        # print(head_dict['cookie'])
        m = re.search("PHPSESSID=66qepujvqe1lksqkj2koosfke7;", head_dict['set-cookie'])
        if m:
            print(head_dict)
            return True
    return False


if __name__ == '__main__':
    get_timestamp('2021-10-25T08:43:24.663')
    get_timestamp('2021-10-25T08:43:24.664')

    # base_64 = 'SG9zdDogd3d3LmR1aWJhLmNvbS5jbg0KQ29ubmVjdGlvbjoga2VlcC1hbGl2ZQ0KQWNjZXB0OiB0ZXh0L2h0bWwsYXBwbGljYXRpb24veGh0bWwreG1sLGFwcGxpY2F0aW9uL3htbDtxPTAuOSxpbWFnZS93ZWJwLCovKjtxPTAuOA0KVXBncmFkZS1JbnNlY3VyZS1SZXF1ZXN0czogMQ0KVXNlci1BZ2VudDogTW96aWxsYS9tb2JpbGUgUURSZWFkZXJBbmRyb2lkLzYuMy4zLzI0NC8xMDAwMDE5LzM1NTMwOTA3MjkxNjM5NA0KcWRpbmZvOiBCbzZ5WHZqSFI1YmNKL05qWXNnamlCQjJBQWFCcU8wb1pDMEFiWHFPZzJvTmpvamcrbUdkMTZnMThXdmFTd3htRU9FdDFBSU5IdjB0dWgrYnM5S1YxTUpMZFQ2blJodkU0aHNzYTlaSWM2dVNWbWliSlpkOGhLeHRWT1F1M3EvY1pzWElQYWY0TWR3PQ0KQWNjZXB0LUVuY29kaW5nOiBnemlwLCBkZWZsYXRlDQpBY2NlcHQtTGFuZ3VhZ2U6IHpoLUNOLGVuLVVTO3E9MC44DQpDb29raWU6IHdkYXRhMz1YZVlWZ3lrRWNCYUUxZnBBcTlGaVo0RDU0aGNlUlE5a2JTQ0ZWQlB3ZTFUNFFncFR5bWt3DQpYLVJlcXVlc3RlZC1XaXRoOiBjb20ucWlkaWFuLlFEUmVhZGVyDQoNCg=='
    # print('Is base64?:',is_base64_code(base_64))
    # head_dict, head_list = head_to_dict(base64.b64decode(base_64).decode())
    # print(head_list)
    # print(get_header_lcs(head_list,'request'))
    #
    # gsl = 'RGF0ZTogTW9uLCAxMSBPY3QgMjAyMSAxMTo0Mjo1MCBHTVQNClNlcnZlcjogQXBhY2hlLzIuNC40OCAoV2luNjQpIE9wZW5TU0wvMS4xLjFrIFBIUC84LjAuOA0KWC1Qb3dlcmVkLUJ5OiBQSFAvOC4wLjgNClNldC1Db29raWU6IFBIUFNFU1NJRD1rNXZ0MTA2ZW1oYTNlcGNudDNzNWZ2ODlnZTsgcGF0aD0vDQpFeHBpcmVzOiBUaHUsIDE5IE5vdiAxOTgxIDA4OjUyOjAwIEdNVA0KQ2FjaGUtQ29udHJvbDogbm8tc3RvcmUsIG5vLWNhY2hlLCBtdXN0LXJldmFsaWRhdGUNClByYWdtYTogbm8tY2FjaGUNCkNvbnRlbnQtTGVuZ3RoOiAwDQpLZWVwLUFsaXZlOiB0aW1lb3V0PTUsIG1heD0xMDANCkNvbm5lY3Rpb246IEtlZXAtQWxpdmUNCkNvbnRlbnQtVHlwZTogdGV4dC9odG1sOyBjaGFyc2V0PVVURi04DQoNCg=='
    # gsl_head_dict, gsl_head_list = head_to_dict(base64.b64decode(gsl).decode())
    # print(gsl_head_list)
    # print(get_header_lcs(gsl_head_list, 'response'))
    #
    #
    # anomaly = "IoRN3RMbXxTH/wcFaGmmYsEgRMesgjBH6YWSqIyKb+p+MOu6yEguCGtVseW2g+sr8v/mR6UXJLFOSFTA9sWU609yZR9fSrU24sc1tDM"
    # normal = 'I am an engineer at Huawei. I received Ph.D. degree in computer science from Tsinghua University in 2021. '
    # print("anomaly: entropy is: {0}, IC is {1}".format(cal_entropy(anomaly),cal_coincidence_index(anomaly)))
    # print("normal: entropy is: {0}, IC is {1}".format(cal_entropy(normal), cal_coincidence_index(normal)))


==> intro_for_compression.tex <==

%日志很重要
Logs, which record a vast range of events of services and underlying machines at runtime, are one of the most valuable data sources for large-scale services~\cite{satpathi2018learning}. 
%Logs describe a vast range of events observed by them, to record  services and their underlying machines' states at runtime.
%日志在运维的多个场景中有应用
Logs have been widely applied for monitoring system status~\cite{li2017flap,Khatuya2018ADELEAD}, understanding system events~\cite{he2018identifying}, detecting anomalies~\cite{loganomaly,deeplog,meng2018device}, and predicting failures~\cite{zhang2018prefix}, using machine learning approaches.
%日志这么重要需要对日志存储
The supervised approaches usually need a large number of failures for training.
However, services and underlying machines rarely fail.
Therefore, these approaches need a long period of logs to train the model.
In addition, the unsupervised approaches, which learn as many normal patterns as possible to detect abnormal patterns, are also trained based on long period of logs.
Consequently, services have to store historical logs for a long time.
%Because machine learning methods as well as manual diagnosis method usually 
%Therefore, it is necessary to record and store logs for a long time. 
%日志量很大，存储很困难，需要对其压缩
With the rapid growth of modern services both in size and complexity, the volume of logs has recently witnessed an explosion.
For example, Google and Facebook respectively generate 100 Petabyte and 10 Petabyte of log data per month~\cite{Manogaran2018Human}.
These massive logs, if not properly compressed, will consume immense storage space. 
When a failure occurs, operators tend to traceback the logs of similar failures for quick mitigation.
However, if logs are compressed with traditional methods (\textit{e.g.,} zip, tar) everyday, which is a common practice in modern large scale services, decompressing such a tremendous volume of logs will consume too much time \cite{harnik2013zip}. This, greatly delays the process of failure diagnosis and mitigation.
%Therefore, massive logs need to do compression.
%Besides, operators usually query logs of a special period, which means that they need to decompress historical logs in real-time. However, traditional compression methods ({e.g.}, zip) cannot real-time decompress for given logs. 
%--------------下一段---------------





%日志虽然是非结构化，但是它有一些特点，是机打的，加个图介绍日志特点
We address the above problem based on the following observations.
An unstructured log is essentially ``printf''ed by services and thus follow some specific format: there is a $template$ field sketching out the event and summarizing this one and other similar logs, and a $variable$ field varying from one log to another.
%As can be seen from several example switch logs shown in Figure~\ref{fig:logs}, although logs are unstructured, most logs are in a specific format (template) provided by developers and produced by ``print'' program of systems. 
%Some $constant$ fields are reflecting the event and $variable$ values in logs. The locations of the variables in the logs of the same category are the same. 
Take Figure~\ref{fig:logs} as an example, in $L_1$, ``ae3'' is a $variable$ word, whereas the rest, \textit{i.e.}, ``Interface ..., changed state to up'', is the $template$ field. 
Usually, the number of different templates are much smaller than that of different logs, and in a log the number of variable words are much smaller than that of all the words.
As a result, a log can be easily compressed (matched) to, and quickly decompressed (recovered) from, its template and variables.
In order to (de)compress every log, the template set should be kept up to date.
Consequently, log parsing, which extracts templates from logs, matches logs to templates, and maintains a template set continuously, is a promising direction to efficiently and effectively compress logs.
    
%In other words, unstructured logs contain many redundant information. 
%Log templates can take advantage of the features of logs to compress logs and query (decompress) them in real-time.
%There are some topic model~\cite{jipeng2019short} and sentence compression~\cite{wang2017can} methods in NLP domain. However, these methods aren't accurate for log analysis domain (shows in Figure \ref{fig:template_evaluation}).
%--------------下一段---------------


%现有的zip方法不能有效利用这些信息，运维工程师会经常查询日志，要求实时压缩和解压日志
%变量信息也压缩在里面了
%Traditional compression approaches ({e.g.,}zip) cannot take advantage of the features of logs. 
%Moreover, traditional approaches are not able to real-time decompress for given logs. They are only suitable to save data long-time.
%NLP文档压缩和句子压缩的不合适，例如TFIDF里的IDF值并不适合日志压缩，有些出现数量多的单词并不是不重要的单词。并且有日志只有一个单词不同，这些需要根据日志的格式来设计压缩方式。

%What's more, these methods cannot distinguish logs accurately sometimes. In Figure \ref{fig:logs}, for example, $L1$ has only one different word from $L3$ and $L4$ ($down/up$, $ae3/ae1$). They are enough similar to clustering or extracting same topics, but we should classify $L1$ and $L4$ to the same event ($T1$), and classify $L3$ to another event ($T2$). 
%--------------下一段---------------


\begin{figure}
      \begin{minipage}[h]{1.0\linewidth}
      \centering
      \includegraphics[width = 7.5 cm]{figures/logs.pdf}\\
      \end{minipage}
       \vspace{-1.2 mm}
       \caption{Examples of logs}\label{fig:logs}
     \vspace{-4 mm}
\end{figure}  

%模板提取方法  
%As the procedure shown in Figure \ref{fig:logs}, log templates can extract event information and convert logs into template indexes. 

The automated, rapid and accurate template extraction has been extensively studied, \textit{e.g.}, Spell \cite{spell}, LogSig \cite{logsig} and FT-Tree~\cite{ft-tree}).
On the contrary, to the best of our knowledge, the other two parts of log parsing, \textit{e.g.,} template matching and maintenance, which are of vital importance for log compression, have not yet been studied.
The design of these two parts faces the following challenges.

\noindent 1. \textbf{New types of logs match no existing templates}. 
To (de)compress every log, the template set has to be able to match any log.
Operators continuously conduct software/firmware upgrades on services and underlying machines to introduce new features, fix bugs or improve performance~\cite{zhang2018funnel}, which can generate new types of logs.
These logs, however, cannot match any existing templates, and thus new templates have to be learned.
The template set should be incrementally learned, otherwise, a new template set has to be learned from all the logs, and the huge amounts of historical logs have to be decompressed from the previous template set and rematched to the new template set for log compression.
Considering the large volume of the long-period historical logs, this is a vast amount of work.

\noindent 2. \textbf{Build and maintaining service/machine type specific template set is labor intensive and time consuming.}
Usually, different types of services/machines are different in log syntax/semantics.
For example, a Windows server and a Ubuntu server generate different types of syslogs and have different template sets.
As a result, current log extraction methods typically extract templates and build a template set for each service/machine type.
There are hundreds to thousands of types of services and machines in large-scale services, and thus building and continuous maintaining different template sets for different types of services/machines consumes too much time and resources.

 

%Recent studies have proposed several data-driven approaches for automated template extraction, \textit{e.g.}, Spell \cite{du2016spell}, LogSig \cite{logsig} and FT-Tree~\cite{ft-tree}) in which historical logs are leveraged to do template extraction. 
%As we all know, services can generate new log templates online. However, most existing approaches cannot extract new templates online, which will lead to creating many unmatched logs. 
%Although periodic retraining can solve new templates,  it will confuse history compression logs in our scenario because of generating new template indexes. 
%Therefore, we need an accurate and general template incrementation mechanism to update template at runtime.
%Above all, the unstructured log compression problem faces the following two challenges. 

%Besides, extracting and maintaining a set of templates for each service is time-consuming and labour intensive. There are massive types of services, but current template extraction methods can only learn log templates for a single service. A service-agnositc template extraction method is beneficial and convenient for operators to manage log templates.
%--------------下一段---------------


%%挑战
%\begin{itemize}
%\item Our preliminary investigation demonstrates that traditional compression methods cannot decompress logs in real-time, which means that they cannot query logs in real-time.
%\item In real-time services, services can generate new log templates, but existing template extraction methods cannot address this problem. If existing templates cannot match new logs, theses new logs cannot compress and decompress.
%%只要用大量的日志数据训练模型，得到了一个单词分类器，就可以直接用训练好的分类器对其他公司的日志数据提取模板了
%\item Training and maintaining a set of templates for each service is time consuming and labor intensive. There are many type of services, but existing template extraction methods can only learn log templates for a single service. 
%\end{itemize}

To address the above challenges, in this paper we propose a novel log parsing framework, \name{}, to rapidly match (compress) logs to templates, and incrementally and service/machine-type agnostically maintain a common template set.
To the best of our knowledge, this is the first log parsing approach that combines template extraction, matching, and maintenance.
It learns the features of template words and variable words based on character-level count and context of words, and trains a word classifier to determine whether a word in a log matching no existing template is a variable word or not.

%It distinguishes template fields and variable fields based on comparing templates and historical logs. 
%Then, feature vectors are constructed by character-level count and context of words. And we train a word classifier to detect which is variable words in unmatched logs.


The contribution of our work is as follows. 

%contributions

\begin{itemize}
\item \name{} learns new templates in an incremental manner, and thus only the logs generated after software/firmware upgrades have to be matched to the updated template set, which greatly reduces the amount of work comparing with rematching all the historical logs to templates.
\item Since \name{} is syntax agnostic, it is general to diverse types of services/machines.
In this way, we build and maintain only one template set for all types of services/machines, which saves a lot of time and resources.
\item \name{} can be easily applied for log compression and decompression. It has a comparable compression ratio, and very quick to query specific historical log(s).
%\item %\item LogTIM, to the best of our knowledge, is the first log parsing approach that conside

%We define a complete log parse framework including template extraction, match and  update. For template update, we propose a general log template increment mechanism, LogTIM, which can handle new types of logs. To the best of our knowledge, LogTIM is the first attempt to update templates at runtime. 
%\item We propose an unstructured log compression system, which can rapidly query  a specific logs.  It includes two solutions for short-term storage and long-term storage. %It takes advantage of the redundancy of unstructured logs and utilize templates to compress logs.
%\item We take LogTIM as a service-agnostic template extraction method. It's general to diverse types of services.
\item We have open-sourced \name{} on GitHub\footnote{https://github.com/LogParse/AAAI-1300}, and hope that it can be used for researches.
%\item We evaluate LogReduce and LogTIM with five public log datasets and six template extraction algorithms. 
\end{itemize}

We have conducted extensive experiments using five publicly available datasets and real-world data from a large service provider, demonstrating \name{}'s  performance: service/machine type agnostic, supporting incremental learning, quick in querying specific log(s) from compressed logs.
%We do evaluation LogTIM on five public log datasets.
Specifically, our results show that \name{} achieves nearly parsing 100\% accuracy and 4.6\% compression ratio. 
Additionally, it can query 857,191 logs per second from compressed logs, where tradition methods cost several hours to decompress logs of one day.

%The rest of the paper is organized as follows: 
%Section~\ref{sec:background} provides the background of our problem, and the design of \name{} is shown in Section ~\ref{sec:design}. The evaluation is shown in Section~\ref{sec:evaluation}.
%Finally, we conclude our work in Section~\ref{sec:conclusion}.





==> white.tex <==
Zhou Yi	 
	
电话：	(+86) 185-1904-0115	电子邮件：	archizhouyi@163.com	
Personal Evaluation
·Four and a half years of content operation experience, verified personal account, Zhihu column and several 10w+ articles, 2W+ followers in Red Book
·Proficient in brand marketing of various copywriting and creative event planning, with acute insight of hot topics.
· Proficient in user operation, with experience in building new media from 0-1 and operating 10w+ user-level accounts
·Data analysis specialist, clear business logic, good planning/organizing skills, and meticulous execution
Skills		
Skill in Windows, Mac and other software / proficient in video editing, Photoshop, Illustrator	TOEFL :95	CET6:558
TAL Education Group U.S.	Campus recruitment brand operation	2020.04—2021.11
Content operation: Responsible for the planning, interviews, reports of technical staff and corresponding official account operation
Technical brand building: Build a media matrix of various official accounts including Bilibili.
Increase the followers of public account by 4 times and empower technical campus recruitment. 
Brand EVP construction: Excavate the value of employers and fulfill brand communication strategies. Plan and construct the campus recruitment VI system including corporate videos and websites. Contribute to the publicity of EVP in business groups.
Internal referral operation: Improve the internal referral occupation from 13.8% to 80%, increase the staff participation rate by 4 times, and save 90% of campus recruitment costs. Facilitate the development of the internal referral operation of the group's technical campus recruitment by event planning, internal publicity, and system optimization,
Operating activities: Assist technical groups in the national technical competition and the seminar of the international competition, enhancing the TAL’s technological influence.
Artron Art Group	Content operation	2019.03 – 2020.04  
IP content planning: Plan original course columns and short video, breaking 10w+ views in multiple media platforms. Attract users to the group chat, official account, and mini program to achieve precise e-commerce.
User operation: Investigate users fission activities in platform/group chat, and design various novel activities for users, gaining 11w and 9W users increments, respectively. Build a community operation system to achieve 30% of the platform’s transaction.
Event planning: Develop international and domestic exhibition activities to improve brand influence in multiple channels, achieving precise art user growth and conversion (attract 3,800 followers in 2 days)
Artron Art Group	Branding	2017.04 – 2019.03 
Content planning: Responsible for the planning of art activities, online/offline publicity, and official account operation.
Brand promotion: Responsible for the promotion and media management of Artron Art Center's fashion salon and art activities.
Product planning: Responsible for the R&D and planning of the artist's derivatives, as well as the writing and dissemination of artwork manuscripts.
Education
2012.9-2017.7 	Shandong University	Architecture	Bachelor
Project experience

2020.04 —2021.06 TAL's official account operation & Bilibili construction

Project description: Build a media matrix with official accounts and station B as the main camps, improve the influence of technology brands, and empower recruitment.
Project role: Responsible for the content operation and referral of the official account and station B.
Project achievement: mining the group’s technical staff, creating a technical content library (manufacturing library + media material library), outputting a series of thematic technical manuscripts,
Completed the creative planning of campus recruitment and referral, the fans increased by 4 times

2021.05 –2021.07
Technical campus recruitment of internal referral operation

Project description: Cooperate with 22 technical transfer internships and school recruits to complete the open source of resumes in the internal push channel,
Project role: Increase the referral rate through internal referral and activity operations; expand the influence of internal referral and referral within the company and save recruitment cost.
Project achievement: internal referral accounted for 74.3% of all channels, internal referral accounted for 80% of job postings, saving 90% of the total cost of campus recruitment and publicity, and everyone's job success the cost fell to 7%.

2020.04-2020.10 TAL Employer Brand EVP and Implementation
Project description: Establish an attractive and TAL campus employer brand image, and empower the recruitment of talents on the future campus
Project role: Enhance Employer Brand Expression: Refine attractive TAL campus employer value propositions, and output relevant concepts, norms and views.
Sense VI system; improve technical brand influence: develop related communication strategies, brand activities, employee stories, etc.
Project achievement: Output employer brand EVP referralal materials and referralal films, and deliver technical talents who have completed key colleges and universities.

2019.07-2019.10 "The Quest of the Louvre" and "Deyi KOL talls" IP planning
Project description: Use PGC to attract new users, and promote retention, so as to realize the community's product conversion.
Project role: plan the topic content of the two columns, write dimensionality reduction content, and output interesting articles and Vlogs, set new goals and community points
System, the launch of community activities.
Project achievement: "The Quest of the Louvre" has achieved 1,400 new users in the community, with a transaction volume of platform



